Pixel-Accurate Epipolar Guided Matching

Keypoint matching can be slow and unreliable in challenging conditions such as repetitive textures or wide-baseline views. In such cases, known geometric relations (e.g., the fundamental matrix) can be used to restrict potential correspondences to a narrow epipolar envelope, thereby reducing the search space and improving robustness. These epipolar-guided matching approaches have proved effective in tasks such as SfM; however, most rely on coarse spatial binning, which introduces approximation errors, requires costly post-processing, and may miss valid correspondences. We address these limitations with an exact formulation that performs candidate selection directly in angular space. In our approach, each keypoint is assigned a tolerance circle which, when viewed from the epipole, defines an angular interval. Matching then becomes a 1D angular interval query, solved efficiently in logarithmic time with a segment tree. This guarantees pixel-level tolerance, supports per-keypoint control, and removes unnecessary descriptor comparisons. Extensive evaluation on ETH3D demonstrates noticeable speedups over existing approaches while recovering exact correspondence sets.

==> sec/6_Conclusion.tex <==
\section{Conclusion \& Future Work}

We presented a pixel-accurate epipolar-guided matching method that avoids the discretization errors of existing approaches. By reformulating the problem as a 1D angular interval query from the epipole and solving it with a segment tree, our approach retrieves the exact set of candidates within a user-defined pixel tolerance in logarithmic time. This design offers fine-grained control at the keypoint level, eliminates unnecessary descriptor comparisons, and integrates seamlessly into standard matching pipelines. Experiments on ETH3D demonstrate that our method achieves consistent speedups over prior geometric-guided techniques while preserving all valid correspondences. 
%
While effective in practice, our method has two main limitations: it assumes a finite epipole (epipoles at infinity have not been witnessed during our experiments) and cannot reuse a segment tree for larger tolerances. Since rebuilding adds less than 10\% to execution time, the overhead is minor. Future work will address these cases while also integrating our geometric filtering into learned matching approaches and extending the framework to handle three-view matching.

\newpage

